MmWave 6D Radio Localization with a Snapshot Observation from a Single BS

Accurate and ubiquitous localization is crucial for a variety of applications such as logistics, navigation, intelligent transport, monitoring, control, and also for the benefit of communications. Exploiting millimeter-wave (mmWave) signals in 5G and Beyond 5G systems can provide accurate localization with limited infrastructure. We consider the single base station (BS) localization problem and extend it to 3D position and 3D orientation estimation of an unsynchronized multi-antenna user equipment (UE), using downlink multiple-input multiple-output orthogonal frequency-division multiplexing (MIMO-OFDM) signals. Through a Fisher information analysis, we show that the problem is often identifiable, provided that there is at least one multipath component in addition to the line-of-sight (LoS), even if the position of corresponding incidence point (IP) is a priori unknown. Subsequently, we pose a maximum likelihood (ML) estimation problem, to jointly estimate the 3D position and 3D orientation of the UE as well as several nuisance parameters (the UE clock offset and the positions of IPs corresponding to the multipath). The ML problem is a high-dimensional non-convex optimization problem over a product of Euclidean and non-Euclidean manifolds. To avoid complex exhaustive search procedures, we propose a geometric initial estimate of all parameters, which reduces the problem to a 1-dimensional search over a finite interval. Numerical results show the efficiency of the proposed ad-hoc estimation, whose gap to the Cram\'er-Rao bound (CRB) is tightened using the ML estimation.

==> MyPackages_Myheaders/bio.tex <==
\begin{IEEEbiography}{Mohammad A. Nazari}
Biography text here.
\end{IEEEbiography}

==> MyPackages_Myheaders/cammands_RespLett.tex <==
\newcommand{\MN}[1]{\textcolor{RedOrange}{\footnotesize{\textsf{[Mohammad:~#1]}}}}
\newcommand{\GS}[1]{\textcolor{RedViolet}{\footnotesize{\textsf{[Gonzalo:~#1]}}}}
\newcommand{\PJ}[1]{\textcolor{Magenta}{\footnotesize{\textsf{[Pontus:~#1]}}}}
\newcommand{\HW}[1]{\textcolor{Red}{\footnotesize{\textsf{[Henk:~#1]}}}}
\newcommand{\ColorBlue}[1]{\textcolor{blue}{#1}}
% ------------------------
\DeclareRobustCommand{\Reviewerbox}[2][lightgray!30]{%
\begin{tcolorbox}[
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #2
\end{tcolorbox}
}
\DeclareRobustCommand{\myActionbox}[2][Cyan!20]{%
\begin{tcolorbox}[
        breakable,
        left=0pt,
        right=0pt,
        top=0pt,
        bottom=0pt,
        colback=#1,
        colframe=#1,
        width=\dimexpr\textwidth\relax, 
        enlarge left by=0mm,
        boxsep=5pt,
        arc=0pt,outer arc=0pt,
        ]
        #2
\end{tcolorbox}
}
% ------------------------
\newcounter{Reviewer}
\setcounter{Reviewer}{0}
\newcounter{ReviewerComment}[Reviewer]
\setcounter{ReviewerComment}{0}
\newcommand{\Editor}{\section*{\Large Response to the Editor}\vspace{5mm}}
\newcommand{\Reviewer}{\stepcounter{Reviewer}\bigskip\section*{\Large Response to the Reviewer \theReviewer}\vspace{5mm}}
\renewcommand{\theReviewerComment}{\theReviewer.\arabic{ReviewerComment}} 
\newcommand{\ReviewerComment}[1]{\refstepcounter{ReviewerComment}\bigskip\noindent\Reviewerbox{{\textbf{Comment~R\theReviewerComment:}}~\itshape#1}}
\newcommand{\EditorSummary}[1]{\Reviewerbox{{\itshape#1}}}
\newcommand{\ReviewerSummary}[1]{\Reviewerbox{\itshape#1}}
\newcommand{\Reply}[1]{\begin{adjustwidth}{0.5cm}{0pt}{\textbf{Reply:}~#1}\end{adjustwidth}}
\newcommand{\Action}[1]{\myActionbox{{\textbf{Action:}}~#1}}
% ------------------------
% command for adding prefix R before references
\makeatletter
\renewcommand\@bibitem[1]{\item\if@filesw \immediate\write\@auxout
{\string\bibcite{#1}{R\the\value{\@listctr}}}\fi\ignorespaces}
\def\@biblabel#1{[R#1]}
\makeatother
